Holistically-Attracted Wireframe Parsing: From Supervised to Self-Supervised Learning

This article presents Holistically-Attracted Wireframe Parsing (HAWP), a method for geometric analysis of 2D images containing wireframes formed by line segments and junctions. HAWP utilizes a parsimonious Holistic Attraction (HAT) field representation that encodes line segments using a closed-form 4D geometric vector field. The proposed HAWP consists of three sequential components empowered by end-to-end and HAT-driven designs: (1) generating a dense set of line segments from HAT fields and endpoint proposals from heatmaps, (2) binding the dense line segments to sparse endpoint proposals to produce initial wireframes, and (3) filtering false positive proposals through a novel endpoint-decoupled line-of-interest aligning (EPD LOIAlign) module that captures the co-occurrence between endpoint proposals and HAT fields for better verification. Thanks to our novel designs, HAWPv2 shows strong performance in fully supervised learning, while HAWPv3 excels in self-supervised learning, achieving superior repeatability scores and efficient training (24 GPU hours on a single GPU). Furthermore, HAWPv3 exhibits a promising potential for wireframe parsing in out-of-distribution images without providing ground truth labels of wireframes.

==> authors.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/nxue2.png}}]{Nan Xue} 
is currently a research scientist at Ant Research, affiliated with Ant Group. Previously, from 2020 to 2023, he served as a research associate professor in the School of Computer Science at Wuhan University. He completed his Ph.D. at the LIESMARS (State Key Laboratory of Information Engineering in Surveying, Mapping, and Remote Sensing), Wuhan University, in 2020. From 2018 to 2020, he worked as a visiting Ph.D. student with the iVMCL Group at NC State University. Prior to pursuing his Ph.D., he obtained a B.S. degree from the School of Mathematics and Statistics at Wuhan University in 2014.
His current research focuses on developing robust and general learning systems that incorporate geometric structures such as parsimonious point sets, line segments, wireframes, and planes for image-based 3D perception and reconstruction.
\end{IEEEbiography}


	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/tfwu.jpg}}]{Tianfu Wu}
		is an associate professor in the Department of Electrical and Computer Engineering at NC state university (NCSU), and leads the laboratory for interpretable visual modeling, computing and learning (iVMCL). He received his Ph.D. in statistics from UCLA in 2011.	His research focuses on computer vision, often motivated by the task of building explainable and improvable visual Turing test and robot autonomy through life-long communicative learning. To accomplish his research goals, he is interested in pursuing a unified framework for machines to ALTER (Ask, Learn, Test, Explain and Refine) recursively in a principled way.
	\end{IEEEbiography}
	

	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/song_trans.png}}]{Song Bai} is a Computer Vision Lead in ByteDance/TikTok Singapore, and also holds an appointment as an Adjunct Assistant Professor at the Department of Electrical and Computer Engineering, National University of Singapore. Before that, he was a research fellow at the University of Oxford working with Prof. Philip H.S. Torr. He serves as an Associate Editor of Pattern Recognition and Guest Editor of IEEE Transactions on Pattern Analysis and Machine Intelligence. He has served as Area Chair/SPC of CVPR 2023/2024, NeurIPS 2023, and AAAI 2022. His research interests include computer vision and machine learning. More information can be found on his homepage:~\url{http://songbai.site/}.
	\end{IEEEbiography}
	

	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/wfd-new.pic.jpg}}]{Fu-Dong Wang}
		 is currently a researcher at Ant Group. Prior to that, he worked at Youtu Lab, Tencent. He earned his Ph.D. degree from the State Key Laboratory of Information Engineering in Surveying, Mapping, and Remote Sensing at Wuhan University in 2021. He also holds a B.S. degree in basic mathematics from Wuhan University, which he obtained in 2016. His research interests include neural radiance rendering, 3D human reconstruction, and motion generation.
	\end{IEEEbiography}
	

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/gsxia-1.jpg}}]{Gui-Song Xia}
(M'10-SM'15) received his Ph.D. degree in image processing and computer vision from CNRS LTCI, T{\'e}l{\'e}com ParisTech, Paris, France, in 2011. From 2011 to 2012, he has been a Post-Doctoral Researcher with the Centre de Recherche en Math{\'e}matiques de la Decision, CNRS, Paris-Dauphine University, Paris, for one and a half years.
He is currently working as a full professor in computer vision and photogrammetry at Wuhan University. He has also been working as Visiting Scholar at DMA, {\'E}cole Normale Sup{\'e}rieure (ENS-Paris) for two months in 2018. His current research interests include mathematical modeling of images and videos, structure from motion, perceptual grouping, and remote sensing imaging. He serves on the  Editorial Boards of the journals Pattern Recognition, Signal Processing: Image Communications, and EURASIP Journal on Image \& Video Processing.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/zhang.pdf}}]{Liangpei Zhang}
received the B.S. degree in physics from Hunan Normal University, Changsha,  	China, in 1982, the M.S. degree in optics from the Xi’an Institute of Optics and Precision Mechanics, Chinese Academy of Sciences, Xi’an, China,	in 1988, and the Ph.D. degree in photogrammetry and remote sensing from Wuhan University, Wuhan, China, in 1998. He is currently a Chang-Jiang Scholar Chair Professor with Wuhan University, appointed by
the Ministry of Education of China. He has authored or co-authored over 500 research papers and five books. He holds 15 patents. His research interests include hyper spectral remote sensing, highresolution remote sensing, image processing, and artificial intelligence.
Dr. Zhang was a recipient of the 2010 Best Paper Boeing Award and the 2013 Best Paper ERDAS Award from the American Society of Photogrammetry and Remote Sensing. He serves as a Co-Chair for the series SPIE Conferences on Multispectral Image Processing and Pattern Recognition, the Conference on Asia Remote Sensing, and many other conferences. He serves as an Associate Editor for the IEEE Transactions on Geoscience and Remote Sensing. He is a fellow of IEEE,
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/torr.jpeg}}]{Philip H. S. Torr}
received the PhD degree from Oxford University. After working for another three years at Oxford, he worked for six years for Microsoft Research, first in Redmond, then in Cambridge, founding the vision side of the Machine Learning and Perception Group. He is now a professor at Oxford University. He has won awards from top vision conferences, including ICCV, CVPR, ECCV, NIPS and BMVC. He is a senior member of the IEEE and a Royal Society Wolfson Research Merit Award holder.
\end{IEEEbiography}

==> lastcounters.tex <==
\setcounter{figure}{13}
\setcounter{table}{5}

